Robustness of Random Forest-based gene selection methods

Gene selection is an important part of microarray data analysis because it provides information that can lead to a better mechanistic understanding of an investigated phenomenon. At the same time, gene selection is very difficult because of the noisy nature of microarray data. As a consequence, gene selection is often performed with machine learning methods. The Random Forest method is particularly well suited for this purpose. In this work, four state-of-the-art Random Forest-based feature selection methods were compared in a gene selection context. The analysis focused on the stability of selection because, although it is necessary for determining the significance of results, it is often ignored in similar studies. The comparison of post-selection accuracy in the validation of Random Forest classifiers revealed that all investigated methods were equivalent in this context. However, the methods substantially differed with respect to the number of selected genes and the stability of selection. Of the analysed methods, the Boruta algorithm predicted the most genes as potentially important. The post-selection classifier error rate, which is a frequently used measure, was found to be a potentially deceptive measure of gene selection quality. When the number of consistently selected genes was considered, the Boruta algorithm was clearly the best. Although it was also the most computationally intensive method, the Boruta algorithm's computational demands could be reduced to levels comparable to those of other algorithms by replacing the Random Forest importance with a comparable measure from Random Ferns (a similar but simplified classifier). Despite their design assumptions, the minimal optimal selection methods, were found to select a high fraction of false positives.

==> tabErr.tex <==
\begin{tabular}{r||r|r|r|r}

Method & \Alo & \Gol & \Kha & \Sin \\
\hline



RF-ACE & 18.9 & 6.0 & 0.7 & 12.1 \\
Boruta Ferns depth 1 & 19.0 & 6.0 & 0.7 & 9.8 \\
Boruta Ferns depth 2 & 18.2 & 6.0 & 0.7 & 10.1 \\
Boruta Ferns depth 3 & 18.3 & 6.0 & 0.7 & 9.6 \\
Boruta Ferns depth 4 & 18.3 & 6.0 & 0.7 & 9.8 \\
Boruta Ferns depth 5 & 17.8 & 6.0 & 0.7 & 9.3 \\
Boruta Ferns depth 6 & 18.6 & 6.0 & 0.7 & 9.3 \\
Boruta Ferns depth 7 & 18.6 & 6.0 & 0.7 & 9.6 \\
Boruta RF Gini & 19.0 & 6.0 & 0.7 & 8.8 \\
Boruta RF Raw & 18.1 & 6.0 & 0.7 & 9.3 \\
Boruta RF Norm. & 18.1 & 6.0 & 0.7 & 9.3 \\
RFE Ferns depth 1 & 20.3 & 5.4 & 1.3 & 8.7 \\
RFE Ferns depth 2 & 19.9 & 5.7 & 1.0 & 8.1 \\
RFE Ferns depth 3 & 19.9 & 4.9 & 1.6 & 8.3 \\
RFE Ferns depth 4 & 20.3 & 4.0 & 1.3 & 9.0 \\
RFE Ferns depth 5 & 19.9 & 5.6 & 1.0 & 8.5 \\
RFE Ferns depth 6 & 20.2 & 6.3 & 2.9 & 7.8 \\
RFE Ferns depth 7 & 20.8 & 5.8 & 1.3 & 7.8 \\
RFE RF Gini & 21.9 & 4.1 & 2.5 & 8.6 \\
RFE RF Raw & 20.3 & 6.0 & 1.6 & 7.6 \\
RFE RF Norm. & 22.0 & 5.5 & 2.0 & 7.6 \\
RRF & 20.8 & 14.1 & 14.4 & 16.4 \\
No selection & 21.8 & 9.2 & 1.5 & 10.9 \\

\end{tabular}


